One note in three: a verified census of three deployed AI scribes, and the instrument that counted it

Ambient AI scribes draft clinical notes under the reassurance that a clinician signs every note. We audited three commercial AI scribes on the same 142 consultations: 565 notes from recorded UK primary-care and US ambulatory encounters plus authored scenarios. Twelve discovery passes proposed 13,678 candidate errors; the 5,898 clearing an importance filter went to an adversarial panel of two models from different families, each told to refute what it could, and 618 survived. One note in three (31.3% [27.0, 35.6]) carries a verified failure, concentrated in allergy and medication information, invented patient identity, and history written up as examination on telephone consultations that can contain none. No product was given a patient record; setting aside the two classes a record would have prefilled, invented identity and dates, the rate is 24.8% [20.8, 29.0]. One failure mode did not fit our scheme, drawn from published scribe-error taxonomies: a treatment the clinician retracts, recorded as delivered care. Two clinicians adjudicated blind, disjoint samples: a physician author upheld 20 of 21 findings (95.2% [77.3, 99.2]) and an independent clinician, not an author, 12 of 12 ([75.8, 100]); both judged every sampled refusal genuine. A failure rate depends on the instrument as much as the scribes. With model, evidence and settings fixed, the review instruction alone moves the share of candidates verified from 9.3% to 79.0%, and the reviewing family moves it too: alone at that instruction the gentler flags 54.8% of notes against 27.8%. Between 28% and 97% of sampled notes carry a failure depending on the standard. Published audits disagree among themselves by a margin instrument differences alone can produce: omission is 54-86% of their errors against our 23.1%. We release all 618 findings with transcript-side evidence, every prompt and model version, and the re-runnable pipeline.

==> tables/t2_clusters.tex <==
% T2 - the 17 subcategories. Generated by paper/figures/extract_t1_t2.py from
% paper/figures/t2_clusters.json; do not edit by hand, regenerate.
% Requires \usepackage{booktabs} and \usepackage{array}; \textdegree needs textcomp
% (loaded by default since the 2020 LaTeX kernel).
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.20\linewidth}rrrrrr>{\raggedright\arraybackslash}p{0.10\linewidth}>{\raggedright\arraybackslash}p{0.31\linewidth}@{}}
\toprule
& & \multicolumn{3}{c}{product} & & high & place in &\\
\cmidrule(lr){3-5}
Subcategory & n & A & B & C & consultations & importance & the scheme & example\\
\midrule
Allergy status and medication list omissions & 111 & 19 & 40 & 52 & 33 & 71 & omission & Allergy status was asked and answered in the consultation, and the note documents none while recording a prescription. [PARAPHRASED, Scribe B] \\
Invented patient identity: name and sex & 93 & 10 & 45 & 38 & 34 & 49 & addition / fabrication & The patient's name is inaudible in the transcript, and the note supplies one that is a chemotherapy brand name. [PARAPHRASED, Scribe C] \\
Stated working diagnosis dropped from note & 53 & 53 & 0 & 0 & 22 & 52 & omission & The clinician tells the patient the symptoms suggest gastroenteritis; the note carries the advice that follows from it and no impression at all. [PARAPHRASED, Scribe A] \\
Relative timing converted to invented calendar dates & 44 & 0 & 4 & 40 & 17 & 2 & wrong output / timing & The transcript says 'yesterday' and the note prints a specific calendar date. [PARAPHRASED, Scribe C] \\
Remote consult history written as objective exam & 42 & 0 & 11 & 31 & 10 & 33 & addition / examination provenance & A telephone consultation in which no examination took place, written up with examination findings as observed. [PARAPHRASED, Scribe C] \\
Planned investigations documented as already done & 32 & 4 & 15 & 13 & 11 & 21 & wrong output / modality hardening & The transcript has an ECG still to be arranged with reception; the note records it as performed in clinic today. [PARAPHRASED, Scribe C] \\
Fabricated/flipped symptom qualifiers (sleep, timing, location) & 28 & 0 & 14 & 14 & 12 & 11 & addition / fabrication & The note reports the symptoms as affecting sleep, which the consultation never mentions. [PARAPHRASED, Scribe B] \\
Diabetes lab values distorted and re-provenanced & 21 & 6 & 11 & 4 & 4 & 6 & wrong output / dose value & The transcript gives a recalled HbA1c of about 7.7 per cent and the note records 7.0 per cent. [PARAPHRASED, Scribe B] \\
Fabricated calendar year for vague onset date & 21 & 0 & 12 & 9 & 2 & 0 & wrong output / timing & 'Last December' becomes December 2025, a year the consultation never states and the patient's stated age contradicts. [PARAPHRASED, Scribe C] \\
Phantom counselling and unasked negative history & 20 & 0 & 11 & 9 & 8 & 4 & addition / fabrication & The clinician asks whether a previous doctor discussed the risks of aspirin; the note records that the advice was given in this consultation. [PARAPHRASED, Scribe C] \\
Family-history relative and lineage misassignment & 18 & 0 & 0 & 18 & 1 & 4 & wrong output / attribution & A cancer the transcript places in the maternal grandmother is recorded against the patient's mother. [PARAPHRASED, Scribe C] \\
Dropped work-absence and sick-note plan elements & 16 & 11 & 5 & 0 & 8 & 3 & omission & The clinician tells the patient not to go into work until this is sorted out, and the plan omits it. [PARAPHRASED, Scribe A] \\
False denials of swelling/redness & 16 & 0 & 6 & 10 & 4 & 7 & wrong output / negation & The patient reports inflamed knees and the examination finds swelling and redness; the note records both as denied. [PARAPHRASED, Scribe C] \\
Alternative options recorded as issued prescriptions/orders & 14 & 6 & 0 & 8 & 4 & 13 & wrong output / modality hardening & A choice offered between two antibiotics is listed as two issued prescriptions. [PARAPHRASED, Scribe C] \\
Unmeasured or corrupted values entered as objective vitals & 13 & 0 & 1 & 12 & 4 & 7 & addition / examination provenance & A temperature the patient took at home enters the vitals as an observed measurement, its value corrupted to an implausible 13.7\textdegree{}C. [PARAPHRASED, Scribe C] \\
Retracted device captured as delivered care & 11 & 7 & 4 & 0 & 1 & 5 & no published category & The clinician retracts the thumb spica in the next breath and substitutes a wrist brace; the note records the spica as applied. [PARAPHRASED, Scribe A] \\
Red-flag safety-netting downgraded to routine follow-up & 10 & 6 & 1 & 3 & 4 & 7 & wrong output / negation & Sudden weight gain is given as a red flag warranting urgent contact, and the note attaches it to the routine booking instruction. [PARAPHRASED, Scribe A] \\
\bottomrule
\end{tabular}
\caption{\textbf{All 17 subcategories, from the 618 verified findings.} The first two tiers of the taxonomy were fixed before the findings were sorted; the third is discovered from the data. We embed each verified finding's description, project it with UMAP and cluster by density with HDBSCAN, then label each cluster in one call (full recipe and parameters in Appendix A). 563 of the 618 verified findings fall in a cluster and 55 are left unassigned. The count carries measured instability: re-running the same recipe under UMAP seeds 42, 43 and 44 gives 17, 20 and 21 clusters with largely the same boundaries (pairwise adjusted Rand index 0.667, 0.707 and 0.808, mean 0.727, where 1.0 is identical groupings), so the count is stable only to within a few. Columns A, B and C count findings rather than notes; high importance is the verification panel's own rating, out of the cluster's n. Placement in the fixed top two tiers is one call for the whole cluster, so cluster sizes do not sum to the top-level class totals in Section 3.2; 16 of the 17 clusters place under a tier-2 category and one has no category in our scheme, whose classes come from the published taxonomies. Examples are paraphrased from our own finding descriptions rather than quoted from the notes. Tier-1 and tier-2 names are plain-language forms of the released scheme's category identifiers; Table~\ref{tab:checkability} carries each hunted category's description.}
\label{tab:clusters}
\end{table*}

